Near-Optimal Offline Reinforcement Learning via Double Variance Reduction

We consider the problem of offline reinforcement learning (RL) -- a well-motivated setting of RL that aims at policy optimization using only historical data. Despite its wide applicability, theoretical understandings of offline RL, such as its optimal sample complexity, remain largely open even in basic settings such as \emph{tabular} Markov Decision Processes (MDPs). In this paper, we propose Off-Policy Double Variance Reduction (OPDVR), a new variance reduction based algorithm for offline RL. Our main result shows that OPDVR provably identifies an $\epsilon$-optimal policy with $\widetilde{O}(H^2/d_m\epsilon^2)$ episodes of offline data in the finite-horizon stationary transition setting, where $H$ is the horizon length and $d_m$ is the minimal marginal state-action distribution induced by the behavior policy. This improves over the best known upper bound by a factor of $H$. Moreover, we establish an information-theoretic lower bound of $\Omega(H^2/d_m\epsilon^2)$ which certifies that OPDVR is optimal up to logarithmic factors. Lastly, we show that OPDVR also achieves rate-optimal sample complexity under alternative settings such as the finite-horizon MDPs with non-stationary transitions and the infinite horizon MDPs with discounted rewards.

==> sections/formulation.tex <==
% !TEX root = ../Uniform_OPE_icml.tex



Starting with non-stationary, finite horizon tabular MDP $M=(\mathcal{S},\mathcal{A},r,P,d_1,H)$ and any non-stationary policy $\pi$ (as explained in Section~\ref{sec:introduction}), we can characterize more intermediate quantities under the distribution induced by $M$ and $\pi$. Similar to \cite{yin2020asymptotically}, we denote $d^\pi_t(s_t,a_t)$ the induced joint state-action distribution at time $t$ and $d^\pi_t(s_t)$ the marginal state distribution, satisfying $d^{\pi}_t(s_t,a_t)=d^{\pi}_t(s_t)\cdot \pi(a_t|s_t)$. The initial distribution is always set to be identical for any policy $\pi$ (\textit{i.e.} $d^\pi_1=d_1$ $\forall \pi\in\Pi$) as policy will only take effect when state is given so it will never change the initial state. Also, we use $P^\pi_{j,i}:=P^\pi_{i+1,i}\cdot P^\pi_{i+2,i+1}\cdot...\cdot P^\pi_{j,j-1} \in\mathbb{R}^{S\times S}, \;\forall j>i$ to denote the multi-step state transition probabilities from step $i$ to step $j$, where $P^\pi_{t+1,t}(s^\prime|s)=\sum_a P_{t+1,t}(s^\prime|s,a)\pi_t(a|s)$. The connection between marginal state distribution vector ${d}_t^\pi(\cdot)$ and the state transition $P^\pi_{t,t-1}$ is characterized by
$
{d}_t^\pi  = {P}^{\pi}_{t,t-1} {d}_{t-1}^\pi
$. If we overload the notation $P^\pi_{t,t-1}$ to represent the state-action transition $P^\pi_{t,t-1}(s',a'|s,a):=P_t(s'|s,a)\pi_t(a'|s')$, then the marginal state-action vector $d^\pi_t(\cdot,\cdot)\in\R^{S\times A}$ satisfies the same expression $d^\pi_t=P^\pi_{t,t-1}d^\pi_{t-1}$. Note here we abuse $d^\pi_t$ and $P^\pi_{t,t-1}$ by assigning them with either state or state-action meaning to avoid notation redundancy. Lastly, we define the quantity
$
v^\pi_t(s)=\E_\pi[\sum_{t'=t}^H r_{t'}|s_t=s] 
$
and the Q-function
$Q^\pi_t(s,a)=\E_\pi[\sum_{t'=t}^H r_{t'}|s_t=s,a_t=a]$ for all $t=1,...,H$.

\noindent\textbf{Error measures for OPE.} Most works directly use \textit{Mean Square Error} (MSE) $\E[(\widehat{v}^\pi-v^\pi)^2]$ as the criterion for measuring OPE methods \cite{thomas2016data,thomas2015safe,thomas2017predictive,farajtabar18a}, or equivalently, by proposing unbiased estimators and discussing its variance \cite{jiang2016doubly}. In contrast, we consider bounding the absolute difference between $v^\pi$ and $\widehat{v}^\pi$ with high probability, \textit{i.e.} $|\widehat{v}^\pi-v^\pi|\leq \epsilon_\mathrm{prob}$ \textit{w.h.p.}. Generally speaking, high probability bound can be seen as a stricter criterion compared to MSE  since 
\begin{align*}
\E[(\widehat{v}^\pi-v^\pi)^2]&=\E[(\widehat{v}^\pi-v^\pi)^2\mathds{1}_{E}]+\E[(\widehat{v}^\pi-v^\pi)^2\mathds{1}_{E^c}]\\
&\leq \epsilon_\mathrm{prob}(\delta)^2\cdot (1-\delta)+H^2\cdot \delta,
\end{align*}
where $E$ is the event that $\epsilon_\mathrm{prob}$ error holds and $\delta$ is the failure probability.\footnote{Here we also assume $v^\pi,\widehat{v}^\pi$ is bounded by $H$ in this illustration. } As a result, if both $\delta$ and $\epsilon_\mathrm{prob}(\delta)$ can be controlled small, then the high probability bound implies a result for MSE bound.

\subsection{Uniform convergence problems}\label{sec:problems}
\noindent\textbf{Uniform convergences in off-policy evaluation.} For any given error $\epsilon>0$, we want to know if there is an estimator $\widehat{v}^\pi$ such that the absolute difference between $\widehat{v}^\pi$ and $v^\pi$ can be uniformly bounded below $\epsilon$ for all $\pi\in\Pi$ with high probability. In other words, the uniform convergence in OPE asks: can we obtain 
\[
\sup_{\pi\in\Pi}|\widehat{v}^\pi-v^\pi|<\epsilon,
\]
with high probability? Furthermore, a more important question is: how many sample of episodes do we need at least in order to achieve this accuracy? Or equivalently, can uniform convergence in OPE be derived efficiently?

The policy class $\Pi$ we considered here consists of all the non-stationary deterministic policies and in this case $|\Pi|=A^{HS}$. By the standard theoretical results in tabular reinforcement learning, there exists at least one deterministic policy that is optimal \cite{sutton2018reinforcement}.\footnote{An optimal policy satisfies $\pi^\star=\argmax_{\pi}v^\pi$, with $\pi$ chosen from any policy, deterministic or stochastic. } Therefore, the deterministic policy class is rich enough for evaluating any learning algorithm (\textit{e.g.} Q-value iteration in \citet{sidford2018near}) that wants to learn to the optimal policy and deriving uniform convergence over this policy class is high nontrivial. 



\noindent\textbf{Local uniform convergence in the neighborhood of empirical optimal policy.} Given empirical MDP $\widehat{M}$ (\textit{i.e.} the transition kernel is replaced by $\widehat{P}_t(s_{t+1}|s_{t},a_{t}):=n_{s_{t+1},s_{t},a_{t}}/n_{s_{t},a_{t}}$ if $n_{s_t,a_t}>0$ and $0$ otherwise, where $ n_{s_{t},a_{t}}$ is the number of visitations to$(s_t,a_t)$ among all $n$ episodes\footnote{Similar definition holds for $n_{s_{t+1},s_{t},a_{t}}$.}), it is convenient to learn the empirical optimal policy $\widehat{\pi}^\star:=\argmax_{\pi}\widehat{v}^\pi$ since the full empirical transition $\widehat{P}$ is known. Classical methods like Policy Iteration (PI) and Value Iteration (VI) can be leveraged for finding $\widehat{\pi}^\star$. This observation allows us to ask the following interesting question: can uniform convergence over all policies that are close to the empirical optimal policy be obtained efficiently? Mathematically, let
$
\Pi_1:=\lbrace \pi:s.t.\; ||\widehat{v}^\pi_t-\widehat{v}^{\widehat{\pi}^\star}_t ||_\infty\leq\epsilon_\mathrm{opt},\;\forall t=1,...,H\rbrace
$ with $\epsilon_\mathrm{opt}\geq0$ pre-specified, can we efficiently obtain 
\[
\sup_{\pi\in\Pi_1} |\widehat{v}^\pi-v^\pi|<\epsilon
\]
with high probability? Our answers to these two questions are carefully presented in Section~\ref{sec:results}.

\subsection{Assumptions}
We present some mild regularity assumptions that are required for considering uniform convergence OPE problem.
\begin{assumption}[Bounded rewards]\label{assume1}
	$\forall \;t=1,...,H$ and $i=1,...,n$, $0\leq r^{(i)}_t\leq 1$.
\end{assumption}
\vspace{-5pt}
MDP with bounded reward is a common assumption in most RL literature. The upper bound can be replaced by any $R_\mathrm{max}$ by scaling and the boundedness will become essential for applying concentrate inequalities.



\begin{assumption}[Sufficient exploration]\label{assume2}
Logging policy $\mu$ obeys that $\min_{t,s_t}d^\mu_t(s_t)>0$, for any state $s_t$ that is ``accessible''.
\end{assumption}
\vspace{-5pt}

State $s_t$ is ``accessible'' means there exists a policy $\pi$ so that $d^\pi_t(s_t)>0$. If for any policy $\pi$ we always have $d^\pi_t(s_t)=0$, then state $s_t$ can never be visited in the given MDP. Assumption~\ref{assume2} simply says logging policy $\mu$ have the right to explore all ``accessible'' states. This assumption is required for the consistency of off-policy evaluation estimator. As a short comparison, off-policy learning problems (\textit{e.g.} off-policy policy optimization in \citet{liu2019off})  only require $d_t^\mu(s_t)>0$ for any state $s_t$ satisfies $d^{\pi^\star}_t(s_t)>0$.  

\begin{assumption}[Near uniformity]\label{assume3}
We assume $d_m:=\min_{t,s_t ,a_t} d^\mu_t (s_t , a_t )>\Omega(1/SA)$, for any state $s_t$ that is ``accessible''  .
\end{assumption}

\vspace{-5pt}

If logging policy $\mu$ only has tiny probability on certain ``accessible'' $(s_t,a_t)$ and this $(s_t,a_t)$ happens to have large reward, then we will need huge amount of off-policy samples in order to correct evaluate the target policy which chooses $\pi_t(s_t)=a_t$. In this case, uniform convergence over all deterministic policies can never be achieved in a sample efficient way. This assumption actually shows the difference between uniform convergence in OPE and standard OPE with a fixed target policy as standard OPE need another bounded weights assumption for that specific target policy \cite{xie2019towards,yin2020asymptotically}.

Last but not least, even though our target policy class is deterministic, by above assumptions the logging policy $\mu$ is always stochastic.  

\subsection{method}


The method we use for doing off-policy evaluation in uniform convergence problem is the empirical model approximation estimator. EMA uses off-policy data to build the empirical estimators for both the transition dynamic and the expected reward and then substitute the related components in real value function by its empirical counterparts. First recall for any target policy $\pi$, by definition:

\vspace{-10pt}

{\small
\[
\begin{aligned}
v^\pi&=\sum_{t=1}^H\E_\pi\left[ r_{t}\right] =\sum_{t=1}^H\sum_{s_t}d^\pi_t(s_t)r^\pi_t(s_t)\\
&=\sum_{t=1}^H\sum_{s_t}{d}^\pi_t(s_t)\sum_{a_t}{r}_t(s_t,a_t)\pi(a_t|s_t)\\
&=\sum_{t=1}^H\sum_{s_t,a_t}{d}^\pi_t(s_t,a_t){r}_t(s_t,a_t)\\
\end{aligned} 
\]
}

\vspace{-10pt}

 where both the marginal state and marginal state-action transitions satisfy $d^\pi_t=P^\pi_td^\pi_{t-1}$. To provide an estimator for this quantity, EMA directly construct empirical estimates for $\widehat{P}_{t+1}(s_{t+1}|s_{t},a_{t})$ and $\widehat{r}_t(s_t,a_t)$ as: 
 
 \vspace{-15pt}
 
{\small
	%\begin{equation}\label{eq:tabular_MIS_construction}
	%\hspace{-3.5mm}
	\begin{align*}
	\widehat{P}_{t+1}(s_{t+1}|s_{t},a_{t})&=\frac{\sum_{i=1}^n\mathbf{1}[(s^{(i)}_{t+1},a^{(i)}_t,s^{(i)}_t)=(s_{t+1},s_{t},a_{t})]}{n_{s_{t},a_{t}}},\\
	\widehat{r}_t(s_t,a_t)&=\frac{\sum_{i=1}^n r_t^{(i)}\mathbf{1}[(s^{(i)}_t,a^{(i)}_t)=(s_t,a_t)]}{n_{s_t,a_t}},
	\end{align*}
	%\end{equation}
}

\vspace{-15pt}

 where $\widehat{P}_{t+1}(s_{t+1}|s_{t},a_{t})=0$ and $\widehat{r}_t(s_t,a_t)=0$ if $n_{s_t,a_t}=0$ (recall $n_{s_t,a_t}$ is the empirical visitation frequency to state-action $(s_t,a_t)$ at time $t$) and then the estimates for state transition $\widehat{P}^\pi_t$ and average state reward $\widehat{r}^\pi_t$ are defined as:
%\begin{equation}\label{eq:tabular_MIS_construction2}
\begin{align*}
\widehat{P}^\pi_t(s_t|s_{t-1})&=\sum_{a_{t-1}}\widehat{P}_t(s_t|s_{t-1},a_{t-1})\pi(a_{t-1}|s_{t-1}),\\
\widehat{r}^\pi_t(s_t)&=\sum_{a_t}\widehat{r}_t(s_t,a_t)\pi(a_t|s_t).
\end{align*}
%\end{equation}
%\vspace{-5pt}
The initial distribution is also constructed using empirical estimator $\widehat{d}_1^\pi(s_1)=n_{s_1}/n$. Based on the construction, the empirical marginal state and state-action transition follows $\widehat{d}^\pi_t=\widehat{P}^\pi_t\widehat{d}^\pi_{t-1}$ and the final estimator for $v^\pi$ is:
{\small
\begin{equation}\label{eqn:estimated_value}
\widehat{v}_\mathrm{EMA}^\pi=\sum_{t=1}^H\sum_{s_t}\widehat{d}^\pi_t(s_t)\widehat{r}^\pi_t(s_t)=\sum_{t=1}^H\sum_{s_t,a_t}\widehat{d}^\pi_t(s_t,a_t)\widehat{r}_t(s_t,a_t).
\end{equation}
}
\vspace{-15pt}

In contrast to model-free methods like importance sampling estimators, EMA estimator is model-based method since it uses plug-in estimators ($\widehat{d}^\pi_t$ and $\widehat{r}^\pi_t$) for each model components (${d}^\pi_t$ and ${r}^\pi_t$). Also, unlike many OPE methods that explicitly uses importance sampling weights, EMA does not require the exact form of logging policy $\mu$ therefore it can be applied to a wider range of tabular reinforcement learning problems, as pointed by \citet{yin2020asymptotically}.




==> sections/method.tex <==

% !TEX root = ../Uniform_OPE_icml.tex

\subsection{Tabular Marginalized Importance Sampling Estimator}

\textbf{We stick with the tabular marginalized importance sampling estimator (TMIS). }

In addition to the non-stationary, finite horizon tabular MDP $M=(\mathcal{S},\mathcal{A},r,T,d_1,H)$ (where $S:=|\mathcal{S}|<\infty$ and $A:=|\mathcal{A}|<\infty$), non-stationary logging policy $\mu$ and target policy $\pi$ in Section~\ref{sec:preliminary}, we denote $d^\mu_t(s_t,a_t)$ and $d^\pi_t(s_t,a_t)$ the induced joint state-action distribution at time $t$ and the state distribution counterparts $d^\mu_t(s_t)$ and $d^\pi_t(s_t)$, satisfying $d^{\pi}_t(s_t,a_t)=d^{\pi}_t(s_t)\cdot \pi(a_t|s_t)$.\footnote{For $\mu$, $d^{\mu}_t(s_t,a_t)=d^{\mu}_t(s_t)\cdot \mu(a_t|s_t)$.} The initial distributions are identical $d_1^\mu=d^\pi_1=d_1$. Moreover, we use $P^\pi_{i,j}\in\mathbb{R}^{S\times S}, \;\forall j<i$ to represent the state transition probability from step $j$ to step $i$ under policy $\pi$, where $P^\pi_{t+1,t}(s^\prime|s)=\sum_a P_{t+1,t}(s^\prime|s,a)\pi_t(a|s)$.  The marginal state distribution vector ${d}_t^\pi(\cdot)$ satisfies
${d}_t^\pi  = {P}^{\pi}_{t,t-1} {d}_{t-1}^\pi,$

Historical data $\mathcal{D}=\left\lbrace (s_t^{(i)},a_t^{(i)},r_t^{(i)})\right\rbrace_{i\in[n]}^{t\in[H]} $ was obtained by logging policy $\mu$ and we can only use $\mathcal{D}$ to estimate the value of target policy $\pi$, \emph{i.e.} $v^\pi$. Suppose we only assume knowledge about $\pi(a|s)$ for all $(s,a)\in\mathcal{S}\times\mathcal{A}$ and \emph{do not observe} $r_t(s_t,a_t)$ for any actions other than the noisy immediate reward $r_t^{(i)}$ after observing $s_t^{(i)},a_t^{(i)}$. 

\begin{assumption}[Bounded rewards]\label{assume1}
	 $\forall \;t=1,...,H$ and $i=1,...,n$, $0\leq r^{(i)}_t\leq R_{\max}$.
\end{assumption}
The bounded reward assumption can be relaxed to:  $\exists R_{\max},\sigma<+\infty$ such that $0\leq \mathbb{E}[r_t|s_t,a_t,s_{t+1}]\leq R_{\max}$, $\mathrm{Var}[r_t|s_t,a_t,s_{t+1}]\leq \sigma^2$ (as in \citet{xie2019towards}), for achieving Cramer-Rao lower bound. However, the boundedness will become essential for applying concentrate inequalities in deriving high probability bounds.

\begin{assumption}\label{assume2}
	Logging policy $\mu$ obeys $d_m:=\min_{t,s_t}d^\mu_t(s_t)>0$.
\end{assumption}
This assumption is always required for the consistency of off-policy evaluation estimator. 

\begin{assumption}[Bounded weights]\label{assume3}
	$\tau_s:=\max_{t,s_t}\frac{d^\pi_t(s_t)}{d^\mu_t(s_t)}<+\infty$ and $\tau_a:=\max_{t,s_t,a_t}\frac{\pi(a_t|s_t)}{\mu(a_t|s_t)}<+\infty$.
\end{assumption}
Assumption~\ref{assume3} is also necessary for discrete state and actions, as otherwise the second moments of the importance weight would be unbounded and the MSE of estimators will become intractable . The bound on $\tau_s$ is natural since $\tau_s\leq \max_{t,s_t}\frac{1}{d^\mu_t(s_t)}=\frac{1}{\min_{t,s_t}d^\mu_t(s_t)}=\frac{1}{d_m}$ and it's finite by the Assumption~\ref{assume2}; similarly, $\tau_a<\infty$ is also automatically satisfied if $\min_{t,s_t,a_t}\mu(a_t|s_t)>0$.  

\subsection{Tabular-MIS estimator}

Marginalized importance sampling directly estimates
the marginalized state visitation distribution $\widehat{d}_t$ and defines the MIS estimator:

\begin{equation}\label{MIS_def}
\widehat{v}^\pi_{MIS} =\frac{1}{n}\sum_{i=1}^n\sum_{t=1}^H\frac{\widehat{d}^\pi_t(s_t^{(i)})}{\widehat{d}^\mu_t(s^{(i)}_t)}\widehat{r}^\pi_t(s^{(i)}).
\end{equation}
and $\widehat{d}^\mu_t(\cdot)$ is directly estimated using the empirical mean, \emph{i.e.} $\widehat{d}^\mu_t(s_t):=\frac{1}{n}\sum_i \mathbf{1}(s_t^{(i)}=s_t):=\frac{n_{s_t}}{n}$ whenever $n_{s_t}>0$ and $\widehat{d}^\pi_t(s_t)/\widehat{d}^\mu_t(s_t)=0$ when $n_{s_t}=0$. Then the MIS estimator \eqref{MIS_def} becomes:
\begin{equation}\label{MIS}
\widehat{v}^\pi_{MIS}=\sum_{t=1}^H\sum_{s_t}\widehat{d}^\pi_t(s_t)\widehat{r}^\pi_t(s_t)
\end{equation}

\paragraph{Construction of \TMIS .} 
  
We can construct empirical estimates for $\widehat{P}_{t+1}(s_{t+1}|s_{t},a_{t})$ and $\widehat{r}_t(s_t,a_t)$ as: 
{\small
\begin{equation}\label{eq:tabular_MIS_construction}
%\hspace{-3.5mm}
\begin{aligned}
\widehat{P}_{t+1}(s_{t+1}|s_{t},a_{t})&=\frac{\sum_{i=1}^n\mathbf{1}[(s^{(i)}_{t+1},a^{(i)}_t,s^{(i)}_t)=(s_{t+1},s_{t},a_{t})]}{n_{s_{t},a_{t}}}\\
\widehat{r}_t(s_t,a_t)&=\frac{\sum_{i=1}^n r_t^{(i)}\mathbf{1}[(s^{(i)}_t,a^{(i)}_t)=(s_t,a_t)]}{n_{s_t,a_t}},\\
\end{aligned}
\end{equation}
}
where we set $\widehat{P}_{t+1}(s_{t+1}|s_{t},a_{t})=0$ and $\widehat{r}_t(s_t,a_t)=0$ if $n_{s_t,a_t}=0$, with $n_{s_t,a_t}$ the empirical visitation frequency to state-action $(s_t,a_t)$ at time $t$. The corresponding estimation of $\widehat{P}_{t+1}(s_{t+1}|s_{t},a_{t})$ and $\widehat{r}_t(s_t,a_t)$ are defined as:

\begin{equation}\label{eq:tabular_MIS_construction2}
\begin{aligned}
\widehat{P}^\pi_t(s_t|&s_{t-1})=\sum_{a_{t-1}}\widehat{P}_t(s_t|s_{t-1},a_{t-1})\pi(a_{t-1}|s_{t-1}),\\
\widehat{r}^\pi_t(s_t)&=\sum_{a_t}\widehat{r}_t(s_t,a_t)\pi(a_t|s_t),\;\widehat{d}^\pi_t=\widehat{P}^\pi_t\widehat{d}^\pi_{t-1}. 
\end{aligned}
\end{equation}




%\red{However, model-based approaches are not well-understood even in tabular setting.  Some discussions and summary of the understanding of tabular methods are here: \url{http://nanjiang.cs.illinois.edu/files/cs598/note3.pdf}
%In particular, check the "Simulation Lemma", and check out the various ``naive approaches'' to analyze the model-based methods.}



==> sections/proof_sketch.tex <==
\section{Proof Sketch}
\label{sec:proof_s}


